The Compressor-Retriever Architecture for Language Model OS

Recent advancements in large language models (LLMs) have significantly enhanced their capacity to aggregate and process information across multiple modalities, enabling them to perform a wide range of tasks such as multimodal data querying, tool usage, web interactions, and handling long documents. These capabilities pave the way for transforming LLMs from mere chatbots into general-purpose agents capable of interacting with the real world. This paper explores the concept of using a language model as the core component of an operating system (OS), effectively acting as a CPU that processes data stored in a context window, which functions as RAM. A key challenge in realizing such an LM OS is managing the life-long context and ensuring statefulness across sessions, a feature limited by the current session-based interaction paradigm due to context window size limit. To address this, we introduce compressor-retriever, a model-agnostic architecture designed for life-long context management. Unlike other long-context solutions such as retrieval-augmented generation, our approach exclusively uses the base model's forward function to compress and retrieve context, ensuring end-to-end differentiability. Preliminary experiments demonstrate the effectiveness of this architecture in in-context learning tasks, marking a step towards the development of a fully stateful LLM OS. Project repo available at: https://github.com/gblackout/LM-OS

==> parts/algorithms.tex <==
\SetKwInput{KwInit}{Init}
\begin{algorithm}[t]
\caption{RLHF}
\SetAlgoLined
\KwIn{Reward Model $RM$, NL-perturbed-FOL-rule pairs $\cD = \{\anB{\vx, \vx_{\hat{R}}}_i\}_{i=1}^n$}
\KwInit{The remote $GPT$, Actor $\pi_\theta$ and critic $C_\omega$, experience set $\cE=\emptyset$}

\While{True}{

    \BlankLine

    \tcp{Make experience}
    \For{$i=1\to N$}{
        Sample $\vx, \vx_{\hat{R}} \sim \cD $
        
        Take actions $A = \{a_1, a_2, .., a_T\} \gets \pi_\theta(a_t|\vx, \vx_{\hat{R}})$

        \BlankLine
        \BlankLine
        
        Concatenate the prompts $\vx^* \gets \vx + \vx_{\hat{R}} + A$

        Get response $\vx_R \gets GPT(\vx^*)$

        Parse the rule $R \gets Parser(\vx_R)$

        \BlankLine
        \BlankLine

        \tcp{Only one reward for the whole episode!}
        Get reward $r \gets RM(R)$
        
        \tcp{Estimate the value only for the last action!}
        Last state $s_T \gets \vx + \vx_{\hat{R}} + A_{<T}$
        
        Get value estimates $v = C_\omega(a_T|s_T)$
        
        Compute advantage $adv = r - v$

        \BlankLine
        \BlankLine
        
        Add experience $\cE.add\brB{\anB{s_T, A, r, v, adv}}$
    }

    \BlankLine
    \BlankLine

    \tcp{Policy gradient update on $\pi_\theta$}
    Update $\theta$ with $\nabla \sum_i^N \log \pi_\theta(A|\vx, \vx_{\hat{R}}) * adv_i$

    \BlankLine

    \tcp{Square loss update on $C_\omega$}
    Update $\omega$ with $\nabla \sum_i^N \brB{r_i - v_i}^2$
}


\label{algo:overview}
\end{algorithm}

==> parts/cfg_grammar.tex <==

\ttt{S} -> \ttt{F}   |   \ttt{Q}   \ttt{F}

\ttt{Q} -> \ttt{QUANT}   \ttt{VAR} | \ttt{QUANT} \ttt{VAR} \ttt{Q}

\ttt{F} -> `$\neg$' `(' \ttt{F} `)' | `(' \ttt{F} `)' | \ttt{F} \ttt{OP} \ttt{F} | \ttt{L}

\ttt{OP} -> `$\oplus$' | `$\lor$' | `$\land$' | `$\to$' | `$\leftrightarrow$'

\ttt{L} -> `$\neg$' \ttt{PRED} `(' \ttt{TERMS} `)' | \ttt{PRED} `(' \ttt{TERMS} `)'

\ttt{TERMS} -> \ttt{TERM} | \ttt{TERM} `,' \ttt{TERMS}

\ttt{TERM} -> \ttt{CONST} | \ttt{VAR}

\ttt{QUANT} -> `$\forall$' | `$\exists$'

==> parts/correction-max-n-step-breakdown-wrapfig.tex <==


\begin{wrapfigure}{l}{0.4\textwidth}
    \centering

    \vspace{-.2cm}
    
    \begin{minipage}{0.4\textwidth}        
        \begin{minipage}{\textwidth}
            \centering            
            \captionof{table}{RLHF correction performance vs. Max \# generations.}
            \label{tab:steps-choice}
            \resizebox{\columnwidth}{!}{%
            \begin{tabular}{@{}llclclclcl@{}}
            \toprule
             & \multicolumn{1}{c}{\multirow{2}{*}{Metrics}} & \multicolumn{8}{c}{Max \# Generations} \\ \cmidrule(l){3-10} 
             & \multicolumn{1}{c}{}                         & 1   &    & 3   &    & 5   &    & 10     &   \\ \midrule
             & FOL BLEU                                     & 0.357   &    & 0.373   &    & 0.375   &    & 0.381  &   \\
             & FOL LE                                       & 0.822   &    & 0.831   &    & 0.834   &    & 0.835  &   \\ \bottomrule
            \end{tabular}%
            }
        \end{minipage}
        
        \vspace{.1cm}
        
        \begin{minipage}[b]{0.49\textwidth}
            \centering
            \includegraphics[trim={0 0cm 1.5cm 1.3cm},clip,width=\textwidth]{figs/new_binned_LE.pdf}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.49\textwidth}
            \centering
            \includegraphics[trim={0 0cm 1.5cm 1.3cm},clip,width=\textwidth]{figs/new_binned_bleu.pdf}
        \end{minipage}
        \captionof{figure}{\method-7B correction performance averaged over corresponding GPT-3.5 LE and BLEU scores.}
        \label{fig:binned-scores}   
    \end{minipage}
    
    \vspace{-.5cm}
    
\end{wrapfigure}



==> parts/dataset_stats_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{Statistics of \dataset, LogicNLI, and FOLIO datasets.}
\label{tab:dataset_stats}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccccccccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Dataset}} & \multirow{2}{*}{Source}                                   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\#NL-FOL\\ pairs\end{tabular}} & \multicolumn{2}{c}{NL}                                                                                        &  & \multicolumn{9}{c}{FOL}                                                                                                                              \\ \cmidrule(l){4-15} 
\multicolumn{1}{c}{}                         &                                                           &                                                                           & \begin{tabular}[c]{@{}c@{}}Vocab\\ size\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ \#words\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}Avg.\\ \#literals\end{tabular} & $\forall$ & $\exists$ & $\neg$ & $\land$ & $\lor$ & $\to$ & $\leftrightarrow$ & $\oplus$ \\ \midrule
FOLIO$^3$                                    & Expert & 2K                                                                        & 5105                                                 & 10.4                                                   &  & 2.1                                                       & 1111      & 182       & 421    & 631     & 167    & 1137  & 17                & 121      \\
LogicNLI$^3$                                 & Synthetic                                                 & 12K                                                                       & 2061                                                 & 13.9                                                   &  & 2.8                                                       & 2783      & 5327      & 10230  & 6590    & 2373   & 8712  & 3288              & 0        \\
\dataset                                     & GPT-4                                                     & 28K                                                                       & 20959                                                & 15.7                                                   &  & 4.6                                                       & 27256     & 1738      & 3443   & 25209   & 5164   & 25212 & 1835              & 1777     \\ \bottomrule
\end{tabular}%
}
\end{table}

==> parts/gpt-binned-stats.tex <==
\begin{figure*}[t]
    \begin{minipage}{\textwidth}
    \begin{minipage}{0.54\textwidth}
        \vspace{0pt}
        \centering
        \captionof{table}{BLEU and the logical equivalence (LE) scores of \method and GPT models on LogicNLI and FOLIO. Direct translation using \method outperforms GPT-3.5 and CoT correction achieves a similar performance as 5-shot GPT-4.}
        \label{tab:main-res-table}
        \resizebox{\columnwidth}{!}{%
        \begin{tabular}{@{}lcclcc@{}}
        \toprule
        \multicolumn{1}{c}{\multirow{2}{*}{Methods}} & \multicolumn{2}{c}{LogicNLI} &  & \multicolumn{2}{c}{FOLIO} \\ \cmidrule(lr){2-3} \cmidrule(l){5-6} 
        \multicolumn{1}{c}{}                         & FOL BLEU       & FOL LE      &  & FOL BLEU     & FOL LE     \\ \midrule
        GPT-3.5 0-shot                                & 0.584          & 0.589       &  & 0.248        & 0.429      \\
        GPT-3.5 5-shot                                & 0.905          & 0.918       &  & 0.341        & 0.767      \\
        GPT-4 0-shot                                  & 0.740          & 0.863       &  & 0.372        & 0.799      \\
        GPT-4 5-shot                                  & 0.913          & 0.989       &  & 0.400        & 0.855      \\ \midrule
        Direct Translation                           & 0.926          & 0.965       &  & 0.372        & 0.818      \\
        Naive Correction                             & 0.934          & 0.970       &  & 0.373        & 0.840      \\
        SFT CoT Correction\yy{remove?}                           & 0.663          & 0.830       &  & 0.332        & 0.730      \\
        RLHF CoT Correction                          & 0.935          & 0.978       &  & 0.385        & 0.849      \\ \bottomrule
        \end{tabular}%
        }
    \end{minipage}    
    \begin{minipage}{0.45\textwidth}
        \centering
        \captionof{table}{RLHF CoT correction performance vs. Max \# generations.}
        \begin{minipage}[t]{0.9\textwidth}
            \centering            
            \label{tab:steps-choice}
            \resizebox{\columnwidth}{!}{%
            \begin{tabular}{@{}llclclclcl@{}}
            \toprule
             & \multicolumn{1}{c}{\multirow{2}{*}{Metrics}} & \multicolumn{8}{c}{Max \# Generations} \\ \cmidrule(l){3-10} 
             & \multicolumn{1}{c}{}                         & 1   &    & 3   &    & 5   &    & 10     &   \\ \midrule
             & FOL BLEU                                     & 0.361   &    & 0.370   &    & 0.384   &    & 0.385  &   \\
             & FOL LE                                       & 0.815   &    & 0.841   &    & 0.846   &    & 0.849  &   \\ \bottomrule
            \end{tabular}%
            }
        \vspace{.2cm}
        \end{minipage}        
        \begin{minipage}[b]{0.49\textwidth}
            \centering
            \includegraphics[trim={0 0cm 1.5cm 1.3cm},clip,width=\textwidth]{figs/binned_LE.pdf}
            % \captionof{figure}{\method correction performance averaged over corresponding GPT3.5 LE score.}
            % \label{fig:binned-LE}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.49\textwidth}
            \centering
            \includegraphics[trim={0 0cm 1.5cm 1.3cm},clip,width=\textwidth]{figs/binned_bleu.pdf}
            % \captionof{figure}{\method correction performance averaged over corresponding GPT3.5 BLEU score.}
            % \label{fig:binned-bleu}
        \end{minipage}
        \captionof{figure}{\method correction performance averaged over corresponding GPT-3.5 LE and BLEU scores.}
        \label{fig:binned-scores}
    \end{minipage}    
\end{minipage}
\end{figure*}

==> parts/llama2-gpt-binned-stats.tex <==
\begin{figure*}[t]
    \begin{minipage}{\textwidth}
    \begin{minipage}{0.6\textwidth}
        \vspace{0pt}
        \centering
        \captionof{table}{BLEU and the logical equivalence (LE) scores of \method and GPT models. In all three benchmarks, \method outperforms GPT-3.5, and achieves similar performance as 5-shot GPT-4 with iterative correction. We skip GPT-4 evaluation on \dataset as it is the model that generates it.}
        \label{tab:main-res-table}
        \resizebox{\columnwidth}{!}{%
        \begin{tabular}{@{}lcccccccc@{}}
        \toprule
        \multicolumn{1}{c}{\multirow{2}{*}{Methods}} & \multicolumn{2}{c}{LogicNLI}          &  & \multicolumn{2}{c}{FOLIO} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{MALLS} \\ \cmidrule(l){2-9} 
        \multicolumn{1}{c}{}                         & \multicolumn{1}{l}{FOL BLEU} & FOL LE &  & FOL BLEU     & FOL LE     & \multicolumn{1}{l}{} & FOL BLEU     & FOL LE     \\ \midrule
        LLaMA2-7B 5-shot                             & 0.697                        & 0.783  &  & 0.288        & 0.654      &                      & 0.459        & 0.506      \\
        LLaMA2-13B 5-shot                            & 0.806                        & 0.867  &  & 0.349        & 0.747      &                      & 0.416        & 0.584      \\
        GPT3.5 0-shot                                & 0.584                        & 0.589  &  & 0.248        & 0.429      &                      & 0.407        & 0.141      \\
        GPT3.5 5-shot                                & 0.905                        & 0.918  &  & 0.341        & 0.767      &                      & 0.497        & 0.648      \\
        GPT4 0-shot                                  & 0.740                        & 0.863  &  & 0.372        & 0.799      &                      & -            & -          \\
        GPT4 5-shot                                  & 0.913                        & 0.989  &  & 0.400        & 0.855      &                      & -            & -          \\ \midrule
        LogicLLaMA-7B Trans.                         & 0.912                        & 0.965  &  & 0.354        & 0.826      &                      & 0.762        & 0.910      \\
        LogicLLaMA-7B Corre.                         & 0.913                        & 0.970  &  & 0.368        & 0.827      &                      & 0.767        & 0.910      \\
        LogicLLaMA-7B RLHF Corre.                    & 0.921                        & 0.979  &  & 0.381        & 0.835      &                      & 0.770        & 0.911      \\
        LogicLLaMA-13B Trans.                        & 0.922                        & 0.978  &  & 0.361        & 0.832      &                      & 0.765        & 0.916      \\
        LogicLLaMA-13B Corre.                        & 0.925                        & 0.982  &  & 0.377        & 0.852      &                      & 0.769        & 0.918      \\
        LogicLLaMA-13B RLHF Corre.                   & 0.926                        & 0.985  &  & 0.386        & 0.858      &                      & 0.771        & 0.923      \\ \bottomrule
        \end{tabular}%
        }
    \end{minipage}    
    \begin{minipage}{0.39\textwidth}
        \centering
        \captionof{table}{RLHF correction performance vs. Max \# generations.}
        \begin{minipage}[t]{0.9\textwidth}
            \centering            
            \label{tab:steps-choice}
            \resizebox{\columnwidth}{!}{%
            \begin{tabular}{@{}llclclclcl@{}}
            \toprule
             & \multicolumn{1}{c}{\multirow{2}{*}{Metrics}} & \multicolumn{8}{c}{Max \# Generations} \\ \cmidrule(l){3-10} 
             & \multicolumn{1}{c}{}                         & 1   &    & 3   &    & 5   &    & 10     &   \\ \midrule
             & FOL BLEU                                     & 0.361   &    & 0.370   &    & 0.384   &    & 0.385  &   \\
             & FOL LE                                       & 0.815   &    & 0.841   &    & 0.846   &    & 0.849  &   \\ \bottomrule
            \end{tabular}%
            }
        \vspace{.2cm}
        \end{minipage}        
        \begin{minipage}[b]{0.49\textwidth}
            \centering
            \includegraphics[trim={0 0cm 1.5cm 1.3cm},clip,width=\textwidth]{figs/binned_LE.pdf}
            % \captionof{figure}{\method correction performance averaged over corresponding GPT3.5 LE score.}
            % \label{fig:binned-LE}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.49\textwidth}
            \centering
            \includegraphics[trim={0 0cm 1.5cm 1.3cm},clip,width=\textwidth]{figs/binned_bleu.pdf}
            % \captionof{figure}{\method correction performance averaged over corresponding GPT3.5 BLEU score.}
            % \label{fig:binned-bleu}
        \end{minipage}
        \captionof{figure}{\method correction performance averaged over corresponding GPT-3.5 LE and BLEU scores.\yy{why bleu drops faster}\yy{make it wrapfig}}
        \label{fig:binned-scores}
    \end{minipage}    
\end{minipage}
\end{figure*}

==> parts/main-res-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{BLEU and logical equivalence (LE) scores of LLMs. In all three benchmarks, \method outperforms GPT-3.5, and achieves similar performance as 5-shot GPT-4 with iterative correction. We skip GPT-4 evaluation on \dataset as it is the model that generates it.}
\label{tab:main-res-table}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Methods}} & \multicolumn{2}{c}{LogicNLI}          &  & \multicolumn{2}{c}{FOLIO} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{MALLS} \\ \cmidrule(l){2-9}
\multicolumn{1}{c}{}                         & \multicolumn{1}{l}{FOL BLEU} & FOL LE &  & FOL BLEU     & FOL LE     & \multicolumn{1}{l}{} & FOL BLEU     & FOL LE     \\ \midrule
LLaMA2-7B 5-shot                             & 0.697                        & 0.783  &  & 0.288        & 0.654      &                      & 0.459        & 0.506      \\
LLaMA2-13B 5-shot                            & 0.806                        & 0.867  &  & 0.349        & 0.747      &                      & 0.416        & 0.584      \\
GPT3.5 0-shot                                & 0.584                        & 0.589  &  & 0.248        & 0.429      &                      & 0.407        & 0.141      \\
GPT3.5 5-shot                                & 0.905                        & 0.918  &  & 0.341        & 0.767      &                      & 0.497        & 0.648      \\
GPT4 0-shot                                  & 0.740                        & 0.863  &  & 0.372        & 0.799      &                      & -            & -          \\
GPT4 5-shot                                  & 0.913                        & 0.989  &  & 0.400        & 0.855      &                      & -            & -          \\ \midrule
LogicLLaMA-7B Trans.                         & 0.912                        & 0.965  &  & 0.354        & 0.826      &                      & 0.762        & 0.910      \\
LogicLLaMA-7B Corre.                         & 0.913                        & 0.970  &  & 0.368        & 0.827      &                      & 0.767        & 0.910      \\
LogicLLaMA-7B RLHF Corre.                    & {\textcolor{red}{0.923}}                        & {\textcolor{red}{0.979}}  &  & {\textcolor{red}{0.378}}        & {\textcolor{red}{0.841}}      &                      & {\textcolor{red}{0.774}}        & {\textcolor{red}{0.920}}      \\
LogicLLaMA-13B Trans.                        & 0.922                        & 0.978  &  & 0.361        & 0.832      &                      & 0.765        & 0.916      \\
LogicLLaMA-13B Corre.                        & 0.925                        & 0.982  &  & 0.377        & 0.852      &                      & 0.769        & 0.918      \\
LogicLLaMA-13B RLHF Corre.                   & {\textcolor{red}{0.927}}                        & {\textcolor{red}{0.986}}  &  & {\textcolor{red}{0.384}}        & {\textcolor{red}{0.858}}      &                      & {\textcolor{red}{0.778}}        & {\textcolor{red}{0.924}}      \\ \bottomrule
\end{tabular}%
}
\end{table}

==> parts/perturb-operations-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{The list of all atomic perturbations.}
\label{tab:perturb-operations}
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
\multicolumn{1}{c}{Operation Type} & \multicolumn{1}{c}{Subtypes} & \multicolumn{1}{c}{Original}                             & \multicolumn{1}{c}{Perturbed}                     \\ \midrule
\multirow{4}{*}{Label Change}      & Change Predicate             & $\tblue{P}(A) \land R(B)$                                & $\tred{R}(A) \land R(B)$                          \\
                                   & \multirow{2}{*}{Change Term} & \multirow{2}{*}{$\forall \tblue{x}\;\; P(x) \land P(B)$} & $\forall \tred{y} \;\; P(x) \land P(B)$           \\
                                   &                              &                                                          & $\forall x \;\; P(x) \land P(\tred{x})$     \\
                                   & Change Operator              & $\forall x \;\; P(x) \;\tblue{\land}\; P(B)$                 & $\forall x \;\; P(x) \;\tred{\lor}\; P(B)$            \\ \midrule
\multirow{4}{*}{Insert}            & \multirow{2}{*}{Insert Term} & \multirow{2}{*}{$\forall x \;\; P(x) \land P(B)$}        & $\forall x \; \tred{\exists y} \;\; P(x) \land P(B)$ \\
                                   &                              &                                                          & $\forall x \;\; P(x) \land P(\tred{x, }\;B)$        \\
                                   & Insert Negation              & $P(A) \land P(B) \land P(C)$                             & $P(A) \land \tred{\neg(}P(B) \land P(C)\tred{)}$  \\
                                   & Insert  Formula              & $P(A) \land P(B)$                                        & $P(A) \land P(B) \;\tred{\to R(C)}$                 \\ \midrule
\multirow{4}{*}{Delete}            & \multirow{2}{*}{Delete Term} & $\tblue{\forall x} \; \forall y \;\; P(x) \land R(x, y)$ & $\forall y \;\; P(x) \land R(x, y)$               \\
                                   &                              & $\forall x \; \forall y \;\; P(x) \land R(\tblue{x, }\;y)$ & $\forall x \; \forall y \;\; P(x) \land R(y)$     \\
                                   & Delete Negation              & $\tblue{\neg(}P(A) \land P(B)\tblue{)}$                  & $\neg(P(A) \land P(B))$                           \\
                                   & Delete Formula               & $P(A) \;\tblue{\land}\; \tblue{P(B)}\; \land P(C)$                     & $P(A) \land P(C)$                                 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> parts/perturbation_and_truth_table_le.tex <==
\begin{figure*}[t]
    \begin{minipage}{\textwidth}
    \begin{minipage}{0.59\textwidth}
        \vspace{0pt}
        \centering
        \captionof{table}{The list of all atomic perturbations.}
        \label{tab:perturb-operations}
        \resizebox{\columnwidth}{!}{%
        \begin{tabular}{@{}llll@{}}
        \toprule
        \multicolumn{1}{l}{Operation Type} & \multicolumn{1}{c}{Subtypes} & \multicolumn{1}{c}{Original}                             & \multicolumn{1}{c}{Perturbed}                     \\ \midrule
        \multirow{4}{*}{Label Change}      & Change Predicate             & $\tblue{P}(A) \land R(B)$                                & $\tred{R}(A) \land R(B)$                          \\\cdashline{3-4}
                                           & \multirow{2}{*}{Change Term} & \multirow{2}{*}{$\forall \tblue{x}\;\; P(x) \land P(B)$} & $\forall \tred{y} \;\; P(x) \land P(B)$           \\
                                           &                              &                                                          & $\forall x \;\; P(x) \land P(\tred{x})$     \\\cdashline{3-4}
                                           & Change Operator              & $\forall x \;\; P(x) \;\tblue{\land}\; P(B)$                 & $\forall x \;\; P(x) \;\tred{\lor}\; P(B)$            \\ \midrule
        \multirow{4}{*}{Insert}            & \multirow{2}{*}{Insert Term} & \multirow{2}{*}{$\forall x \;\; P(x) \land P(B)$}        & $\forall x \; \tred{\exists y} \;\; P(x) \land P(B)$ \\
                                           &                              &                                                          & $\forall x \;\; P(x) \land P(\tred{x, }\;B)$        \\\cdashline{3-4}
                                           & Insert Negation              & $P(A) \land P(B) \land P(C)$                             & $P(A) \land \tred{\neg(}P(B) \land P(C)\tred{)}$  \\\cdashline{3-4}
                                           & Insert  Formula              & $P(A) \land P(B)$                                        & $P(A) \land P(B) \;\tred{\to R(C)}$                 \\ \midrule
        \multirow{4}{*}{Delete}            & \multirow{2}{*}{Delete Term} & $\tblue{\forall x} \; \forall y \;\; P(x) \land R(x, y)$ & $\forall y \;\; P(x) \land R(x, y)$               \\
                                           &                              & $\forall x \; \forall y \;\; P(x) \land R(\tblue{x, }\;y)$ & $\forall x \; \forall y \;\; P(x) \land R(y)$     \\\cdashline{3-4}
                                           & Delete Negation              & $\tblue{\neg(}P(A) \land P(B)\tblue{)}$                  & $\neg(P(A) \land P(B))$                           \\\cdashline{3-4}
                                           & Delete Formula               & $P(A) \;\tblue{\land}\; \tblue{P(B)}\; \land P(C)$                     & $P(A) \land P(C)$                                 \\ \bottomrule
        \end{tabular}%
        }
    \end{minipage}    
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[trim={0 6.7cm 14cm 0},clip,width=\textwidth]{figs/truth-table-le.pdf}
        \vspace{-.6cm}
        \captionof{figure}{Example of computing the Logical Equivalence score, 7/8=0.875.}
        \label{fig:truth-table-le}
    \end{minipage}    
\end{minipage}
\end{figure*}

==> parts/prompt-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\caption{List of prompt templates used for prompting GPT4 for NL-FOL pairs.}
\label{tab:prompt-table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule
\begin{tabular}[c]{@{}l@{}}System\\ prompt\end{tabular}               & \begin{tabular}[c]{@{}l@{}}I want to create a dataset for translating natural language (NL) statements into first-order logic (FOL) rules. \\ You will help me to create a diverse set of NL-FOL pairs.\\ \\ For natural language (NL) generation, you should:\\     1. Come up with a statement stating either complex or simple real-world commonsense facts\\     2. The statements are meaningful, and diverse from each other\\ \\ For FOL rule generation:\\     1. You SHOULD USE the following logical operators: $\oplus$ (either or), $\lor$ (disjunction), \\         $\land$ (conjunction), $\to$ (implication), $\forall$ (universal), $\exists$ (existential), $\neg$ (negation), \\         $\leftrightarrow$ (equivalence)\\     2. You *SHOULD NEVER USE* the following symbols for FOL: "\!", "$\neq$", "\%", "="\\     3. The literals in FOL SHOULD ALWAYS have predicate and entities, e.g., "Rounded(x, y)" or "City(guilin)";\\         expressions such as "y = a $\lor$ y = b" or "a $\land$ b $\land$ c" are NOT ALLOWED\\     4. The FOL rule SHOULD ACCURATELY reflect the meaning of the NL statement\\     5. You SHOULD ALWAYS put quantifiers and variables at the beginning of the FOL\\     6. You SHOULD generate FOL rules with either: (1) no variables; (2) one variable "x"; (3) two variables "x", \\         "y"; or (4) three variables "x", "y" and "z"\\ \\ Generation Format: you SHOULD ALWAYS generate the NL and FOL pairs in the following format\\ """\\ --- NL:\\ \{your generated NL\}\\ ---\\ --- FOL:\\ \{your generated FOL\}\\ ---\\ """\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}l@{}}Initial \\ FOLIO \\ Few-shot \\ examples\\ prompt\end{tabular} & \begin{tabular}[c]{@{}l@{}}--- NL:\\ If someone is entire, then he is not serious, and vice versa. \\ --- FOL:\\ $\exists$x entire(x) $\leftrightarrow$ $\neg$serious(x)\\ \\ --- NL: \\ If there is at least one people who is both not excited and not timid, then Jonathan is elderly.\\ --- FOL:\\ $\forall$x ($\neg$excited(x) $\land$ $\neg$timid(x)) $\to$ elderly(Jonathan)\\ \\ --- NL: \\ Someone who is eithor not fresh or entire is always not serious.\\ --- FOL:\\ $\forall$x ($\neg$concerned(x) $\lor$ fresh(x)) $\to$ entire(John)\\ \\ --- NL: \\ If Nathalie is not blue, then Collier is entire.\\ --- FOL:\\ $\neg$blue(Nathalie) $\to$ entire(Collier)\\ \\ --- NL: \\ Someone is courteous and not elderly if and only if he is not excited and not various.\\ --- FOL:\\ $\exists$x (courteous(x) $\land$ $\neg$elderly(x)) $\leftrightarrow$ ($\neg$excited(x) $\land$ $\neg$various(x))\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \midrule
\begin{tabular}[c]{@{}l@{}}Negative \\ N-gram\\ prompt\end{tabular}   & \begin{tabular}[c]{@{}l@{}}They DO NOT involve concepts and terms (and the synonyms) such as "considered","person","either","water",\\ "if it has","if it is","it has a","is considered a","A person is"\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \midrule
\multirow{2}{*}{FOL prompts}                                          & They are {[complex | simple]} statements involving at least {[1 | 2 | 3]} logical variables                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \cmidrule(l){2-2} 
                                                                      & The statement involves diverse logical operators such as logical negation, logical xor and disjunction                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \midrule
\begin{tabular}[c]{@{}l@{}}Break-down \\ prompt\end{tabular}          & {[IMPORTANT]} AVOID making long predicate names like "MoonShinesAtNight","SunShinesDuringDay"                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> parts/sankey_diagram.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[trim={0cm 5.9cm 0cm 0cm},clip,width=0.85\linewidth]{figs/sankey_diagram_snnipet.pdf}
    \caption{Snippet from the top 200 frequent FOL term pairs in \dataset (for full version see Appendix~\ref{app:dataset_app}). Many terms are associated with a wide range of other terms, which suggests the rules are semantically and contextually diverse.}
    %\es{trimmed this and put the full version in appendix}}
    %\es{maybe you could just keep the left column of this (plant, book, bird) and crop the rest out, then rotate it 90' clockwise. it will save you so much space, then put the full version of it in the appendix}}
    \label{fig:sankey-small}
\end{figure}

==> parts/sankey_diagram_full.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[trim={0 0 9cm 0},clip,width=\linewidth]{figs/sankey_diagram.pdf}
    \caption{Top 200 frequent FOL term pairs in \dataset. Many terms are associated with a wide range of other terms, which suggests the rules are semantically and contextually diverse.}
    \label{fig:sankey}
\end{figure}

==> parts/seg-mask-arch-combined-fig.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}{\textwidth}
    \begin{minipage}{0.34\textwidth}
        \centering
        \includegraphics[trim={0 9cm 20.5cm 0},clip,width=\linewidth]{figs/segmented-attn-mask.pdf}
        % \vspace{-.6cm}
        \captionof{figure}{Segmented attention mask.}
        \label{fig:segmented-attention-mask}
    \end{minipage}
    \hfill
    \begin{minipage}{0.65\textwidth}
        \centering
        \includegraphics[trim={0 6.7cm 6.5cm 0},clip,width=\textwidth]{figs/architecture.pdf}        
        \captionof{figure}{Overview of compressor-retriever architecture.}
        \label{fig:arch}
    \end{minipage}    
\end{minipage}
\end{figure*}

==> parts/sft-rlhf-arch-and-truth-table.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}{0.9\textwidth}
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[trim={0 4.5cm 15.5cm 0},clip,width=\linewidth]{figs/sft-rlhf-overview-tight.pdf}
        % \vspace{-.6cm}
        \captionof{figure}{Overview of the SFT and RLHF training for the iterative correction.}
        \label{fig:sft-rlhf-overview}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\textwidth}
        \centering
        \vspace{.8cm}
        \includegraphics[trim={0 6.7cm 14cm 0},clip,width=\textwidth]{figs/truth-table-le.pdf}        
        \captionof{figure}{Example of computing the Logical Equivalence score, 7/8=0.875.}
        \label{fig:truth-table-le}
    \end{minipage}    
\end{minipage}
\end{figure*}

==> parts/sft-rlhf-arch.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[trim={0 4cm 4.8cm 0},clip,width=0.8\linewidth]{figs/sft-rlhf-overview.pdf}
    \caption{Overview of the SFT and RLHF training for the iterative correction mode of \method.}
    \label{fig:sft-rlhf-overview}
\end{figure}

==> parts/task_summary_table.tex <==
\begin{table}[h]
\centering
\caption{Summary of input, output and objectives of task \textbf{(T1-T4)}}
\label{tab:task-summary-table}
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{@{}lllc@{}}
\toprule
\multicolumn{1}{c}{Task}                                                      & \multicolumn{1}{c}{Input}                                               & \multicolumn{1}{c}{Output}                         & Objective \\ \midrule
\begin{tabular}[c]{@{}l@{}}\textbf{(T1)}\\ Direction Translation\end{tabular} & $\vx_\text{NL}$                                                         & $\vx_\text{FOL}$                                   &     \eq{eq:autoregressive-loss}      \\
\begin{tabular}[c]{@{}l@{}}\textbf{(T2)}\\ Naive Correction\end{tabular} & $[\vx_\text{NL}, \hat{\vx}_\text{FOL}]$                                 & $\vx_\text{FOL}$                                   &  \eq{eq:autoregressive-loss}         \\
\begin{tabular}[c]{@{}l@{}}\textbf{(T3)}\\ SFT Correction\end{tabular} & $[\vx_\text{NL}, \hat{\vx}_\text{FOL}, \hat{\cX}_{\Delta,\text{prev}}]$ & $[\hat{\cX}_{\Delta,\text{corr}}, \vx_\text{FOL}]$ &  \eq{eq:autoregressive-loss}        \\
\begin{tabular}[c]{@{}l@{}}\textbf{(T4)}\\ RLHF Correction\end{tabular} & $[\vx_\text{NL}, \hat{\vx}_\text{FOL}, \hat{\cX}_{\Delta,\text{prev}}]$ & $[\hat{\cX}_{\Delta,\text{corr}}, \vx_\text{FOL}]$ &  \eq{eq:ppo-reward}         \\ \bottomrule
\end{tabular}%
}
\end{table}

==> parts/term_freq_literal_freq.tex <==
\begin{figure*}[h]
    \begin{minipage}{\textwidth}
    \begin{minipage}[b]{0.49\textwidth}
        \centering
        \includegraphics[trim={1.3cm 0cm 0.7cm 1.3cm},clip,width=\textwidth]{figs/term_freq_bar.pdf}
        \captionof{figure}{Top 40 frequent FOL terms (\dataset).}
        \label{fig:term-freq}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.49\textwidth}
        \centering
        \includegraphics[trim={0 0cm 1.5cm 1.3cm},clip, width=\textwidth]{figs/literal_freq_hist.pdf}
        \captionof{figure}{Literal frequency distribution (\dataset).}
        \label{fig:literal-freq}
    \end{minipage}
\end{minipage}
\end{figure*}

==> parts/three_modes_with_examples_fig.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[trim={0 8.1cm 0cm 0},clip,width=\linewidth]{figs/three_modes_of_translation_example_fig_wide.pdf}
    \caption{Input and expected outputs for direct translation, naive correction, and iterative correction.}
    \label{fig:three_modes}
\end{figure}

==> parts/two-modes-translation-fig.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[trim={0 8.1cm 0cm 0},clip,width=\linewidth]{figs/two-correction-examples.pdf}
    \caption{Input and expected outputs for translation and correction.}
    \label{fig:two_modes}
\end{figure}
